Sketching Multidimensional Time Series for Fast Discord Mining

Time series discords are a useful primitive for time series anomaly detection, and the matrix profile is capable of capturing discord effectively. There exist many research efforts to improve the scalability of discord discovery with respect to the length of time series. However, there is surprisingly little work focused on reducing the time complexity of matrix profile computation associated with dimensionality of a multidimensional time series. In this work, we propose a sketch for discord mining among multi-dimensional time series. After an initial pre-processing of the sketch as fast as reading the data, the discord mining has runtime independent of the dimensionality of the original data. On several real world examples from water treatment and transportation, the proposed algorithm improves the throughput by at least an order of magnitude (50X) and only has minimal impact on the quality of the approximated solution. Additionally, the proposed method can handle the dynamic addition or deletion of dimensions inconsequential overhead. This allows a data analyst to consider "what-if" scenarios in real time while exploring the data.

==> insert/alg_aggregate.tex <==
\begin{algorithm}[ht]
% \footnotesize
\scriptsize
    \centering
    \caption{
    Aggregation Algorithm\label{alg:aggregate}}
    \begin{algorithmic}[1]
        \Input{
        group association matrix~$\mathbf{R}$, training time series~$\mathbf{T}_{\text{train}}$, testing time series~$\mathbf{T}_{\text{test}}$}
        \Output{aggregated training time series~$\mathbf{\hat{T}}_{\text{train}}$, aggregated testing time series~$\mathbf{\hat{T}}_{\text{test}}$}
        \Function{Aggregate}{$\mathbf{R}, \mathbf{T}_{\text{train}}, \mathbf{T}_{\text{test}}$}
        \State $\mathbf{T}_{\text{train}}, \mathbf{T}_{\text{test}} \gets \textsc{Normalize}(\mathbf{T}_{\text{train}}, \mathbf{T}_{\text{test}})$
        \State $n_{\text{train}} \gets \textsc{GetTimeSeriesLength}(\mathbf{T}_{\text{train}})$
        \State $n_{\text{test}} \gets \textsc{GetTimeSeriesLength}(\mathbf{T}_{\text{test}})$
        \State $n_g \gets \textsc{GetNumberGroup}(\mathbf{R})$, $m_g \gets \textsc{GetGroupSize}(\mathbf{R})$
        \State $\mathbf{\hat{T}}_{\text{train}} \gets $ zero matrix with size $n_g \times n_{\text{train}}$
        \State $\mathbf{\hat{T}}_{\text{test}} \gets $ zero matrix with size $n_g \times n_{\text{test}}$
        \For{$i \in [0, \cdots, n_g - 1]$}
        \For{$j \in [0, \cdots, m_g - 1]$}
        \If{$j < 0.5 m_g$}
        \State $\mathbf{\hat{T}}_{\text{train}}[i, :] \gets \mathbf{\hat{T}}_{\text{train}}[i, :] + \mathbf{T}_{\text{train}}[\mathbf{R}[i, j], :]$
        \State $\mathbf{\hat{T}}_{\text{test}}[i, :] \gets \mathbf{\hat{T}}_{\text{test}}[i, :] + \mathbf{T}_{\text{test}}[\mathbf{R}[i, j], :]$
        \Else
        \State $\mathbf{\hat{T}}_{\text{train}}[i, :] \gets \mathbf{\hat{T}}_{\text{train}}[i, :] - \mathbf{T}_{\text{train}}[\mathbf{R}[i, j], :]$
        \State $\mathbf{\hat{T}}_{\text{test}}[i, :] \gets \mathbf{\hat{T}}_{\text{test}}[i, :] - \mathbf{T}_{\text{test}}[\mathbf{R}[i, j], :]$
        \EndIf
        \EndFor
        \EndFor
        \State \Return $\mathbf{\hat{T}}_{\text{train}}, \mathbf{\hat{T}}_{\text{test}}$
        \EndFunction
    \end{algorithmic}
\end{algorithm}


==> insert/alg_discord.tex <==
\begin{algorithm}[ht]
    \centering
    \caption{\footnotesize
    Discord Mining Algorithm\label{alg:discord}}
    \footnotesize
    \begin{algorithmic}[1]
        \Input{training time series~$T_{\text{train}}$, testing time series~$T_{\text{test}}$, subsequence length $m$}
        \Output{discord time index~$i_t$, discord score~$s$}
        \Function{FindDiscord}{$T_{\text{train}}, T_{\text{test}}, m$}
        \State $P \gets \textsc{ComputeMatrixProfile}(T_{\text{train}}, T_{\text{test}}, m)$
        \State $i_t \gets \argmax P$, $s \gets \max P$
        \State \Return $i_t$, $s$
        \EndFunction
    \end{algorithmic}
\end{algorithm}


==> insert/alg_normal.tex <==
\begin{algorithm}[ht]
    \centering
    \caption{\footnotesize
    Normalization Algorithm\label{alg:normal}}
    \footnotesize
    \begin{algorithmic}[1]
        \Input{training time series~$\mathbf{T}_{\text{train}}$, testing time series~$\mathbf{T}_{\text{test}}$}
        \Output{training time series~$\mathbf{T}_{\text{train}}$, testing time series~$\mathbf{T}_{\text{test}}$}
        \Function{Normalize}{$\mathbf{T}_{\text{train}}, \mathbf{T}_{\text{test}}$}
        \For{$T^{(i)}_{\text{train}}\in \mathbf{T}_{\text{train}}$, $T^{(i)}_{\text{test}}\in \mathbf{T}_{\text{test}}$}
        \State $\mu \gets \textsc{GetMean}(T^{(i)}_{\text{train}})$
        \State $\sigma \gets \textsc{GetSTD}(T^{(i)}_{\text{train}})$
        \State $T^{(i)}_{\text{train}} \gets \frac{T^{(i)}_{\text{train}} - \mu}{\sigma}$, $T^{(i)}_{\text{test}} \gets \frac{T^{(i)}_{\text{test}} - \mu}{\sigma}$
        \EndFor
        \State \Return $\mathbf{T}_{\text{train}}, \mathbf{T}_{\text{test}}$
        \EndFunction
    \end{algorithmic}
\end{algorithm}


==> insert/fig_mrt_add.tex <==
\begin{figure}[htbp]
\centerline{
\includegraphics[width=0.65\linewidth]{insert/image/fig_mrt_add_1.pdf}
}
\caption{
% \footnotesize
The discords are highlighted with \textcolor{red}{red} and their corresponding nearest neighbors are highlighted with \textcolor{yellow}{yellow}.
The $y$-axis is the number of people entering and exiting the station per hour.
The unusual traffic could be caused by the events hosted in the points of interest around each station.
}
\label{fig:mrt_add}
\end{figure}


==> insert/fig_swat_wadi_exp.tex <==
\begin{figure}[htbp]
\begin{subfigure}[b]{0.65\linewidth}
\centering
\includegraphics[width=\textwidth]{insert/image/fig_swat_exp_0.pdf}
\caption{
\footnotesize
SWaT Dataset.
}
\label{fig:swat_exp}
\end{subfigure}
\begin{subfigure}[b]{0.99\linewidth}
\centering
\includegraphics[width=0.99\textwidth]{insert/image/fig_wadi_exp_0.pdf}
\caption{
\footnotesize
WADI Dataset.
}
\label{fig:wadi_exp}
\end{subfigure}
\caption{
% \footnotesize
The prediction generated from the discord-based method is plotted along side with the ground truth label.
For both datasets, the discord-based method ignores the added noisy dimensions.
}
\label{fig:swat_wadi_exp}
\end{figure}


==> insert/tab_balance_exp.tex <==
\begin{table}[ht]
\centering
\caption{
% \footnotesize
The standard deviation of group size is small after duplicates are removed; therefore, each group holds similar number of members.}
\label{tab:balance_exp}
% \resizebox{0.99\columnwidth}{!}{
\scriptsize
\begin{tabular}{c||cccc}
 & \multicolumn{4}{c}{$n_g$} \\
$m_g$ & 100 & 150 & 200 & 250 \\ \hline \hline
10 & 0.00 & 0.12 & 0.15 & 0.18 \\
15 & 0.20 & 0.25 & 0.27 & 0.30 \\
20 & 0.29 & 0.37 & 0.37 & 0.39 \\
25 & 0.43 & 0.49 & 0.48 & 0.50
\end{tabular}
% }
\end{table}

==> insert/tab_synthetic_rank.tex <==
\begin{table}[ht]
\centering
\caption{
% \footnotesize
% The performance of the approximated time series discord mining algorithm is close to the perfect score (i.e., 1).
The performance of the approximated time series discord mining algorithm.
}
\label{tab:synthetic_rank}
% \resizebox{0.99\columnwidth}{!}{
\scriptsize
\begin{tabular}{c||cccc}
 & \multicolumn{4}{c}{$n_g$} \\
$m_g$ & 100 & 150 & 200 & 250 \\ \hline \hline
10 & 0.87 & 0.89 & 0.89 & 0.82  \\ 
15 & 0.93 & 0.95 & 0.97 & 0.97  \\ 
20 & 0.95 & 0.98 & 0.97 & 0.97  \\ 
25 & 0.98 & 1.00 & 1.00 & 0.99 \\ 
\end{tabular}
% }
\end{table}

==> insert/tab_synthetic_time.tex <==
\begin{table}[ht]
\centering
\caption{
% \footnotesize
Despite the similarity in solution quality, the speedup in throughput relative to the exact solution varies from 3.69 to 9.16 for different hyperparameter settings.}
\label{tab:synthetic_time}
% \resizebox{0.99\columnwidth}{!}{
\footnotesize
\begin{tabular}{c||cccc}
 & \multicolumn{4}{c}{$n_g$} \\
$m_g$ & 100 & 150 & 200 & 250 \\ \hline \hline
10 & 9.1582 & 6.3403 & 4.8155 & 3.9207 \\
15 & 8.7641 & 6.1655 & 4.6943 & 3.8373 \\
20 & 8.4434 & 5.9437 & 4.6079 & 3.7483 \\
25 & 8.1029 & 5.7609 & 4.5132 & 3.6908
\end{tabular}
% }
\end{table}
